Explore and Control with Adversarial Surprise

Unsupervised reinforcement learning (RL) studies how to leverage environment statistics to learn useful behaviors without the cost of reward engineering. However, a central challenge in unsupervised RL is to extract behaviors that meaningfully affect the world and cover the range of possible outcomes, without getting distracted by inherently unpredictable, uncontrollable, and stochastic elements in the environment. To this end, we propose an unsupervised RL method designed for high-dimensional, stochastic environments based on an adversarial game between two policies (which we call Explore and Control) controlling a single body and competing over the amount of observation entropy the agent experiences. The Explore agent seeks out states that maximally surprise the Control agent, which in turn aims to minimize surprise, and thereby manipulate the environment to return to familiar and predictable states. The competition between these two policies drives them to seek out increasingly surprising parts of the environment while learning to gain mastery over them. We show formally that the resulting algorithm maximizes coverage of the underlying state in block MDPs with stochastic observations, providing theoretical backing to our hypothesis that this procedure avoids uncontrollable and stochastic distractions. Our experiments further demonstrate that Adversarial Surprise leads to the emergence of complex and meaningful skills, and outperforms state-of-the-art unsupervised reinforcement learning methods in terms of both exploration and zero-shot transfer to downstream tasks.

==> previous_intro_related.tex <==
\begin{abstract}
Unsupervised reinforcement learning studies how to leverage environment statistics to learn useful behaviors without the cost of reward engineering. However, a central challenge in unsupervised reinforcement learning is to extract behaviors that meaningfully affect the world and cover the range of possible outcomes, without getting distracted by inherently unpredictable, uncontrollable, and stochastic elements in the environment. 
% To this end, we propose a method. Building environment statistics that lead to interesting behaviors is challenging in high-dimensional spaces because of the curse of dimensionality, and is even more difficult in stochastic environments.
%%SL.9.30: OK, so the goal of the above sentence is to clearly state the problem that the current method is solving. But right now, I don't really understand the problem: what does "building environment statistics" mean, and why is it challenging? Perhaps a clearer sentence could look something like this: However, a central challenge in unsupervised reinforcement learning is to extract behaviors that meaningfully affect the world and cover the range of possible outcomes, without getting distracted by inherently unpredictable, uncontrollable, and stochastic elements in the environment. To this end, we propose a method...
To this end, we propose a method to explore and learn skills in high-dimensional, stochastic environments based on an adversarial game between two policies controlling a single 
agent
%%SL.9.30: Note that the word "agent" doesn't mean what you think it means here (FWIW, this is a common mistake). An "agent" is not a little robot, it's something that has agency. It is not a body. So it is correct to say "this is a Q-learning agent" but it is not correct to say "the agent has two arms, two legs, and a head" or "the agent is in grid cell 37". Basically, think agent = computer program
%%AF.10.2 Here I call agent an entity that can affect the world via only one action at a time, I might have several bodies but still one single action that is the product of the two adversarial policies, is there a better wording?
and competing over the amount of observation entropy the agent experiences.
%%SL.9.30: Maybe more explicitly explain what the two agents do, e.g.: In this adversarial game, one of the agents seeks out states that maximally surprise the other agent, while the latter aims to avoid surprise.
The internal competition between the two policies drives the agent to seek out increasingly surprising parts of the environment while learning to gain mastery over them. We show that the resulting agent is able to cover the 
% latent
%%SL.9.30: the use of the word latent here is a bit confusing (I know what you mean, but your reader probably will not)
state space of environments with rich observations and learn complex skills. We show that our method outperforms state-of-the-art unsupervised reinforcement learning methods in terms of coverage and emergence of skills in stochastic and high-dimensional environments. 
%%SL.9.30: Do we want to state anything about exploration here? Or are we intentionally avoiding it? If we have good exploration results, I think it probably does make sense to mention them at least in a secondary capacity...

% Reinforcement learning (RL) provides a framework for learning goal-directed policies given user-specified rewards. However, since designing rewards often requires substantial engineering effort, we are interested in the problem of learning without rewards, where agents must discover useful behaviors in the absence of task-specific incentives. Intrinsic motivation is a family of unsupervised RL techniques which develop general objectives for an RL agent to optimize that lead to better exploration or the discovery of skills. In this paper, we propose a new unsupervised RL technique based on an adversarial game which pits two policies against each other to compete over the amount of surprise an RL agent experiences. The policies each take turns controlling the agent. The Explore policy maximizes entropy, putting the agent into surprising or unfamiliar situations. Then, the Control policy takes over and seeks to recover from those situations by minimizing entropy. The game harnesses the power of multi-agent competition to drive the agent to seek out increasingly surprising parts of the environment while learning to gain mastery over them. We show empirically that our method leads to the emergence of complex skills by exhibiting clear phase transitions. Furthermore, we show both theoretically \---via a latent state space coverage argument\--- and empirically that our method has the potential to be applied to the exploration of stochastic, partially-observed environments. We show that Adversarial Surprise learns more complex behaviors, and explores more effectively than competitive baselines, outperforming intrinsic motivation methods based on active inference, novelty-seeking (Random Network Distillation (RND)), and multi-agent unsupervised RL (Asymmetric Self-Play (ASP)) in MiniGrid, Atari and VizDoom environments.
\end{abstract}

\section{Introduction}

Reinforcement learning methods have attained impressive results across a number of domains (e.g., \cite{berner2019dota,kober2013reinforcement,levine2016end,vinyals2019grandmaster}).

% However, the effectiveness of current methods depends heavily on task-specific rewards \citep{vecerik2017leveraging}. 
However, current RL methods typically require a large number of samples for each new task~\citep{dann2018oracle}. In other areas of machine learning, an effective way to mitigate high data requirements has been the use of unsupervised or self-supervised learning~\citep{}. Similarly, humans and animals seem to be able to learn rich priors from their own experience without being told what to do, and children engage in structured but unsupervised play in part as a way to acquire a functional understanding of the world~\citep{}. Based on this intuition, unsupervised RL methods rely on intrinsic motivation: task-agnostic objectives that incentivize the agent to autonomously explore the world and learn behaviors that can be used to solve a range of downstream tasks with little supervision. A general strategy is to exactly or approximately express this task-agnostic objective in the form of a reward function that uses only environment statistics, and then optimize it using standard RL algorithms. 

% For many tasks, designing dense and informative rewards require significant engineering effort, and sparse rewards make learning slow and difficult \citep{riedmiller2018learning}. 
%%SL.9.30: I slightly tweaked the above, but generally I'm not sure this is particularly compelling motivation -- even if you use unsupervised skills, you still eventually need to design a reward function. That is, unsupervised RL doesn't free you from the need to design a reward function. Could start with something like this: However, current RL methods typically require a large number of samples for each new task~\citep{}. In other areas of machine learning, an effective way to mitigate high data requirements has been the use of unsupervised or self-supervised learning~\citep{}. Similarly, humans and animals seem to be able to learn rich priors from their own experience without being told what to do, and children engage in structured but unsupervised play in part as a way to acquire a functional understanding of the world~\citep{}. Based on this intuition, unsupervised RL methods aim to...
% Yet humans and animals easily learn from their own experience without being constantly told what to do. Unsupervised RL is an emerging field that proposes a more human-like
%%SL.9.30: These kinds of claims tend to be a lightning rod for criticism from just about everyone, I would tone it down.
% way to learn, alleviating the need to design task-specific rewards. Most unsupervised RL methods rely on intrinsic motivation: task-agnostic objectives that incentivize the agent to autonomously explore the world and learn behaviors that can be used to solve a range of downstream tasks with little supervision. A general strategy is to exactly or approximately express this task-agnostic objective in the form of a reward function that uses only environment statistics, and then optimize it using standard RL algorithms. 

However, using environment statistics as the sole reward signal becomes difficult when the agent is acting on high-dimensional spaces (e.g., raw images). As we will see, previous methods exhibit unnatural behaviors when the environment is high-dimensional and stochastic. For example, novelty-seeking or surprise-based methods (e.g., using the prediction error of a dynamics model as reward) can fail to explore an environment that contains local sources of entropy such as a ``noisy TV" \citep{schmidhuber2010formal}. We will show that many previous general unsupervised RL approaches exhibit unnatural behaviors in such environments. A typical failure mode occurs in environments that have rich observations generated by a small number of latent states, characterized by a Block MDP \citep{du2019provably}. These environments often trigger the failure of existing methods to explore all possible latent states. 
%%SL.9.30: I think this paragraph focuses a bit too much on the behavior of prior methods. This seems like it will just make people defensive. We do need to clearly state the challenge that we are trying to address, but this "high-dimensional + stochastic" thing comes across to me as too vague to be convincing. I would recommend going with something more specific, and perhaps closer to what we had before.

Instead of explicitly taking into account the structure of the environment \citep{misra2020kinematic},
%%SL.9.30: This seems like a strawman -- I don't think most prior methods on intrinsic motivation are billed primarily as methods for taking into account the structure of the environment, and it's not clear why this is the logical point of comparison.
we propose a general objective that combines recent advances in unsupervised RL with inspiration from the neuroscience community.
%%SL.9.30: Ehh that's a stretch. It's very vaguely related to one niche area of theoretical neuroscience, almost as an analogy. I don't think this statement will be perceived as that credible.
The free energy principle argues that complex niche-seeking behaviors of biological systems are the result of minimizing long-term average surprise on the system sensors \citep{friston2009free,friston2009reinforcement,friston2016active}. Previous work motivated by this principle has shown that when the environment is entropic, a surprise-minimizing agent can indeed learn behaviors that are useful for downstream tasks \citep{berseth2019smirl}. However, when surprise minimization methods fail when applied to environments where the agent can easily access low-entropy states, because the agent remains in the low-entropy states and is not incentivized to explore the environment to find a better niche. This failure mode is known as the \textit{dark room problem} in the neuroscience community \citep{friston2012free}.
%%SL.9.30: I think this issue might come across as very specific to a particular (slightly weird) class of methods that no one actually uses.

Yet humans do not seem to exhibit the two aforementioned failure modes of unsupervised RL and active inference. We argue that both issues can be solved by finding the right balance between exploration and control. For example, a child in a play room does not just try to toss their toys on the floor in every possible pattern, but instead tries to stack them together, find new uses for parts, or combine them in various interesting ways. In this work, we introduce an unsupervised RL method based on an adversarial game that balances exploration and control, called Adversarial Surprise (AS) (see Figure \ref{fig:intro}). Our method addresses both aforementioned failure modes, and leads to the emergence of complex and interesting behaviors, with no access to external reward. 

% learns to shoot 

% and show both theoretically and empirically that it creates natural behaviors in such environments. 
% [Active inference, Dark room, Balance exploration/control example baby playing, etc...]

%%SL.9.30: Should start by summarizing the key contributions. This is very important, because readers need to have no uncertainty about what is the new novel thing in the paper.
Many performance measures can be used to evaluate an unsupervised RL method.
%%SL.9.30: Above sentence seems fairly meaningless.
We evaluate our method with two performance measures that have been used extensively in previous work. The first measure is coverage of the latent state space. In the Block MDP setting,
%%SL.9.30: probably shouldn't introduce the block MDP stuff here -- without context, readers will have no idea what this is all about.
this is a hard problem since each state can generate a wide range of observations. Theoretically, we prove that our method can fully cover the underlying latent state space of a Block MDP.  Empirical studies support this result, and show that unlike previous state-of-the-art methods including Random Network Distillation (RND) \citep{burda2018exploration}, Asymmetric Self-Play (ASP) \citep{sukhbaatar2017intrinsic}, Adversarially Guided Actor-Critic (AGAC) \citep{flet2021adversarially}, and Surprise Minimizing RL (SMiRL) \citep{berseth2019smirl}, Adversarial Surprise can be used to cover the 
% latent
%%SL.9.30: will be hard for readers to understand why "latent"
state space of a wide range of environments. Our second performance measure is zero-shot transfer, and aims at assessing the ability of our method to learn emergent behaviors that are useful for downstream tasks. We show that balancing exploration and control enables the agent to attain higher performance than prior work in standard benchmarks like Atari and Doom, even \textit{without ever having trained with the game reward}. Videos of our agents show interesting, emergent behaviors in Atari, VizDoom and MiniGrid, and are available on the project website: \url{https://sites.google.com/corp/view/adversarial-surprise/home}.


% novelty-seeking methods (eg. using the prediction error of a dynamics model as reward) can lead to unnatural exploratory behavior when the environment is highly stochastic. A famous example of this phenomena is the noisy TV problem, . Some novelty-seeking methods are explicitly trying to solve the noisy TV problem 


% Many prior works have approached the problem of unsupervised RL as one of pure novelty-seeking, training agents to optimize for surprise in the hopes of facilitating better exploration, which can be helpful for learning downstream tasks. However, current novelty-seeking methods don't always produce the desired explorative behavior. In stochastic environments for example, such methods can suffer from the ``noisy TV" problem where the agent becomes distracted by inherently high-entropy elements \cite{schmidhuber2010formal}. In contrast, some biologically-inspired approaches like active inference suggest that complex human-like behaviors are obtained by minimizing the expected surprise on future observations \citep{friston2009free,friston2009reinforcement,berseth2019smirl}. However, in the absence of an informative observation prior that guide the agent towards interesting behaviors, such methods suffer from the ``dark room" problem \cite{friston2012free}: if what the agent can observe from the environment is not surprising, the agent will not be incentivized to learn any complex behavior. This is especially problematic in partially-observed environments. 
% Yet humans seem to always maintain a tension between optimizing for both novelty and familiarity. For example, a child in a play room does not just try to toss their toys on the floor in every possible pattern, but instead tries to stack them together, find new uses for parts, or combine them in various ways. In the same way, we suggest that the right objective for unsupervised RL should be to actively maintaining a tension between exploration and control. Such method would have the potential to produce increasingly complex and interesting behaviors without the limitations of optimizing for novelty or familiarity alone. 
\begin{figure}[t!]
\centering
\begin{subfigure}{.28\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/intro.png}
  \caption{Adversarial game}
\end{subfigure}\hfil%
\begin{subfigure}{.71\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/grid_filmstrip/grid_filmstrip.png}
  \caption{Explore and Control policy taking turns}
\end{subfigure}\hfil%
\caption{Adversarial Surprise is a multi-agent competition in which two policies take turns controlling an RL agent. The Explore policy acts first, and tries to put the agent into surprising, high entropy states. On its turn, the Control policy tries to minimize surprise by finding familiar, low-entropy, predictable states.
%%MC.5.28: states --> observations ?
Figure (b) shows an example rollout of a game.
In the Explore policy's first turn, it attempts to maximize entropy by remaining in the first room with flashing lights (a \textit{noisy TV} state). When the Control policy takes over, it is able to take an action to control the environment, by flipping the switch to stop the lights from flashing. Therefore, when the Explore policy acts again it moves into the next room; this is predicted by our theoretical results, which show that the Explore policy must maximize entropy over the true state space. During the Control policy's next turn it remains in the dark room. 
This process continues until all of the rooms have been visited.}
\label{fig:intro}
%\vspace{-0.7cm}
% \vspace{-1.5cm}
\end{figure}

% In this paper, we maintain a tension between exploration and control by formulating an adversarial game between two policies, which each take turns sequentially acting for the same RL agent.
% The \textit{Explore} policy is novelty-seeking, and attempts to maximize surprise over the course of the episode, putting the agent into a diverse range of novel states. In turn, the \textit{Control} policy must minimize surprise, by learning to manipulate its environment in order to return to safe and predictable states. 
% When combined, the two adversaries engage in an arms race, repeatedly putting the agent into challenging new situations, then attempting to gain control of those situations. Figure \ref{fig:intro} shows an illustration of the method, including a sample interaction. Rather than simply adding noise to the environment, the Explore policy learns to adapt to the Control policy, and to search for increasingly challenging situations from which the Control policy must recover. Thus our method, \textit{Adversarial Surprise} (AS), leverages the power of multi-agent training to generate a curriculum of increasingly challenging exploration and control problems. We show empirically that the competition between the two policies produces the emergence of increasingly complex observable behaviors in the agent by exhibiting clear phase transitions. Furthermore, we show theoretically and empirically that the increasingly complex control and exploration strategies found by the competing policies enable the efficient exploration of stochastic, partially-observable environments that previous methods optimising for novelty or familiarity alone fail to explore.

% Our main contribution is the Adversarial Surprise (AS) algorithm, an unsupervised RL method to actively maintain a tension between exploration and control which leads to the emergence of increasingly complex behaviors. We derive our method, and perform a theoretical analysis in the recently introduced Block MDP setting \cite{du2019provably} which shows \---via a latent space coverage argument\--- that our method can be applied to the exploration of partially-observed, stochastic environments.  
% We present a practical instantiation based on deep reinforcement learning, and provide an empirical evaluation that compares our approach to recent intrinsic motivation and unsupervised RL techniques. Our results demonstrate that our method induces the emergence of complex behaviors that can be used for both control and exploration. As suggested by our theoretical results, we show empirically that our method can be applied to the exploration of partially-observable, stochastic environments, outperforming previous methods like Random Network Distillation (RND) \cite{burda2018exploration}, Suprise-Minimization RL (SMiRL) \cite{berseth2019smirl} and Asymmetric Self Play (ASP). We also show that AS produces more meaningful behaviors in VizDoom \cite{Kempka2016ViZDoom} and Atari \cite{bellemare2013arcade} without any external reward.

\section{Related Work}

% Our method enables the emergence of complex skills without supervision and thus enters into the budding field of unsupervised RL that we briefly survey below. A common strategy in this field is to formulate a task-agnostic objective that uses environment statistics only and to derive an intrinsic reward that enables exact or approximate optimization of this objective using standard RL algorithms. A recurrent question in this field is the applicability of the skills learned. We will show that our method has the potential to be applied to the exploration of stochastic, partially-observable environments.
%We regroups the intrinsic motivation methods into three categories: knowledge-based, competence-based and data-based.

%%SL.9.30: These are typically called novelty-seeking methods

aquere exploration/covergae ; skills ; multi-agent

\textbf{Novelty-seeking and exploration intrinsic rewards} lead the agent to choose actions that increase its coverage of the environment. A simple way to implement a knowledge-based method is to choose as reward the prediction error of a world model \citep{achiam2017surprise, schmidhuber1991possibility, yamamoto2010curiosity, pathak2017curiosity, burda2018exploration}. A major problem of these simple error-based implementations is that the intrinsic reward can be hacked when the environment contains aleatoric uncertainty, \ie..., such as the example of an agent maximizing a forward model error that get stuck in front of a noisy TV \citep{schmidhuber2010formal}. Several work have proposed solutions to deal with aleatoric uncertainty. A simple fix proposed by previous work consists of modelling only what the agent can control using inverse features, yet this fix can be easily hacked if the aleatoric noise is controllable (e.g., having a remote for the noisy TV). More robust solutions proposed by previous work try to approximate the true information gain using variational Bayes or ensemble disagreement \citep{shyam2019model, pathak2019self,houthooft2016vime}. However, implementing such Bayesian procedures is difficult, because it requires scalable and effective modeling of epistemic uncertainty, which itself is a major open problem with high-dimensional models such as neural networks~\citep{some_survey}. Instead of attempting to directly approximate information gain with Bayesian models, our approach indirectly approximates information gain by utilizing two competing agents. As we will show, this recovers an effective coverage strategy under block MDP assumptions, and performs well in practice.

Another problem with these method is that the asumptoti is not exploratory. REcent work try to directly optimize the state marginal by using particle based method or... Our method comes with the guarantee to asymptotically 

% Yet as we will see these methods suffer from the curse of dimensionality.
%%SL.9.30: Do we compare to these methods? If so, it's fine to have a statement like that. But I don't think this has anything to do with the curse of dimensionality. "Curse of dimensionality" does *not* mean that bad things happen as dimensionality increases, it has a very specific technical meaning: as dimensionality increases, something in the algorithm becomes *exponentially* hard. This is virtually never the case under function approximation, hence I don't think this term is appropriate. Perhaps better phrasing would be something like: However, implementing such Bayesian procedures is difficult, because it requires scalable and effective modeling of epistemic uncertainty, which itself is a major open problem with high-dimensional models such as neural networks~\citep{some_survey}.
% As a consequence, the number of samples necessary to get out of aleatoric noise does not scale with the dimension of the environment.
%%SL.9.30: I would delete this sentence, there is not enough evidence to assert this.
% Instead of maximizing the information gain over the whole environment, which suffers from the curse of dimensionality, our method maximizes the information gain over a low-dimensional structure using a policy actively trying to avoid high-entropic part of the environment causing sample inefficiency. 

%%SL.9.30: I think the spirit of this sentence is fine, but as stated it makes a bunch of implicit claims that are not backed up by evidence. Consider rephrasing along these lines: Instead of attempting to directly approximate information gain with Bayesian models, our approach indirectly approximates information gain by utilizing two competing agents. As we will show, this recovers an effective coverage strategy under block MDP assumptions, and performs well in practice. [or something like that]

% using environment statistics method is  

% A major problem with these methods is that the number of samples the agent need to accurately predict the information gain of an action using the prediction error does not scale well to high-dimensional spaces. It leads in particular to the noisy TV problem where an agent is distracted by 

% % [... Surprise, Inverse Feature, RND, Problem: Noisy TV]

\textbf{Competence-based intrinsic rewards} lead the agent to reach states or learn skills that can be useful for downstream tasks. A common approach is to approximately maximize empowerment, which is defined as the mutual information between the agent's actions or skills and the states and quantities how much control the agent has on the environment \citep{klyubin2005all,salge2014empowerment}. A downside of empowerment-based method is that they don't usually scale to high-dimensional spaces due to the computation of the mutual information, and if they do, it is usually to the detriment of exploration \citep{karl2015efficient,salge2014changing,zhao2020efficient,de2018unified,zhang2020metacure,jaques2019social,mohamed2015variational}.
%%SL.9.30: also DIAYN and DADS? though I'm not sure if the above statement about MI methods is entirely defensible -- while I do actually think it's true, many readers will not understand why it is true

\textbf{Multi-Agent ...} A less theoretically grounded to get competences 
Asymmetric Self-Play (ASP) proposes a less theoretically grounded approach to get diverse and complex skills by setting up a competition between two policies, where one policy tries to imitate the other policy \citep{sukhbaatar2017intrinsic,openai2021asymmetric}. This method belongs to the vast line of work harnessing multi-agent competition to induce emergence of complexity \citep{baker2019emergent,dennis2020emergent,xu2020continual,flet2021adversarially,leibo2019autocurricula,schmidhuber1997s}. As we will see however, ASP fails
%%SL.9.30: why? and doesn't that contradict openai2021asymmetric?
in high-dimensional and stochastic environments. Our method can be seen as the best of both world. On one side, it has an information-theoretic objective that enables learning skills in stochastic environments, but that is still simple enough to be effectively computed.
%%SL.9.30: This all sounded great until I got to "it has an ... but that is still simple". Can we come up with a more obvious explanation for why it is the best of both worlds? E.g., something like this: Like ASP, our method uses a simple two-player game to induce exploration and emergent complexity. However, our objective is general and information-theoretic, focusing on minimization or maximization of surprise rather than reaching specific states, and our theoretical results suggest that this provides a principled approach to maximize coverage in stochastic environments. [though I should say this still sounds a bit unclear, mostly because it doesn't explain why ASP fails, or why our method wouldn't fail in the same way as ASP]
On the other side, our method leverage multi-agent competition to get complex skills despite of the simplicity of the information-theoretic objective. 

% \textbf{Data-driven intrinsic rewards} lead the agent to cover the state space by approximately maximizing the state marginal entropy \citep{hazan2019provably, lee2019efficient}. The state marginal entropy is hard to compute in general, and recent work using nearest neighbor entropy estimators have been proposed \citep{seo2021state, liu2021behavior, mutti2021task}. Unlike these works, one of the policies aim at minimizing its state marginal entropy and we approximate the state marginal entropy using an online density model \citep{berseth2019smirl}. 
%%AF.9.30: Maybe cite these work when presenting the method
%%SL.9.30: I think this paragraph is pretty disconnected from the rest. What I would recommend is to fold the entropy maximization methods into the first paragraph, and then separately address SMiRL together with a discussion of free energy. E.g., something like this:
% The design of the Control agent in our method also draws on ideas from surprise minimization and the free energy theory~\citep{}. In prior work, minimization of surprise has been proposed as a model of intelligent behavior in humans and animals, motivated from the standpoint of seeking out a stable niche within the environment~\citep{}, and prior work on unsupervised RL has explored this as a means to discover skills that stabilize an otherwise chaotic environment in a small range of states~\citep{smirl}. However, such approaches make strong assumptions on the environment itself creating enough stochasticity so that pure surprise minimization leads to interesting behavior. Our method does not make this assumption, since the Explore agent itself drives the Control agent into situations from which surprise minimization is challenging.

% \textbf{Novelty-seeking intrinsic motivation:} One of the most frequently studied forms of intrinsic motivation is novelty-seeking, or curiosity, which can be formulated as maximizing the information gain on the agent's dynamics model of the environment \cite{houthooft2016vime,still2012information,bellemare2016unifying,pathak2017curiosity,schmidhuber1991possibility}. Common intrinsic rewards used to approximate curiosity include surprise \cite{achiam2017surprise, schmidhuber1991possibility, yamamoto2010curiosity, pathak2017curiosity, burda2018exploration} and ensemble disagreement \cite{shyam2019model, pathak2019self}. A novelty-seeking agent is motivated to explore its environment.
% However, na\"{i}vely maximizing surprise leads to methods that are vulnerable to the \textit{noisy TV} problem, where the agent becomes distracted by inherently high-entropy, unpredictable elements in the environment, such as white noise (e.g. static on a TV) \cite{schmidhuber2010formal}.
% In this case, a curious agent will not be able to learn meaningful behaviours. We will show that AS overcomes this problem, and fully explores the state space even when there are highly stochastic elements. 

% \textbf{Surprise minimization and the free energy principle:} Rather than maximizing surprise, the free energy principle \cite{faraji2018balancing,friston2009free,friston2009reinforcement,friston2016active,ueltzhoffer2018deep} proposes that biological agents actually \textit{minimize} long-term average surprise by seeking familiar, stable states, and controlling their environment to make it more predictable.
% Inspired by this idea, \citet{berseth2019smirl} built a surprise-minimizing RL agent, SMiRL, which outperforms curiosity-maximizing methods like ICM \cite{pathak2017curiosity} in high-entropy environments. However, in partially observed or low-entropy environments, surprise minimization is vulnerable to the \textit{dark room} problem: if the agent can simply stay in a highly-predictable part of the environment where nothing happens, it will \cite{friston2012free}. In this scenario, a surprise-minimizing agent cannot learn meaningful behaviors either. AS is designed to avoid this problem, because the Explore policy will not allow the Control policy to remain in a dark room.
% %Curiously, the SMiRL paper revealed that both surprise-minimizing and surprise-maximizing agents can perform better than a vanilla RL baseline \cite{berseth2019smirl},
% %showing that optimizing for either familiarity or novelty can be a useful intrinsic motivation. In this work, we propose a way to combine these seemingly opposing objectives through multi-agent competition.

% \textbf{Empowerment:} The goal of \textit{empowerment} \cite{klyubin2005all,salge2014empowerment} is to maximize the mutual information between the agent's actions and its future states. Empowerment encourages agents to ``keep their options open" by exploring many states, while still maintaining a high degree of control in those states.
% %%[addressed-ish]SL.5.5: The above three sentences can be shortened, and this idea can be communicated in one sentence.
% However, calculating empowerment in high dimensional environments is intractable, leading to various methods for approximating it (e.g., \cite{karl2015efficient,salge2014changing,zhao2020efficient,de2018unified,zhang2020metacure,jaques2019social,mohamed2015variational}). Unfortunately, these methods can also be difficult to get working with high dimensional function approximation \cite{gregor2016variational}. In contrast, we show that Adversarial Surprise works with deep neural networks applied to pixel inputs in Atari environments.%While we do not approximate empowerment, we draw a connection to it which helps provide intuition for our method.
% %efficient empowerment \cite{karl2015efficient}

% \textbf{Emergence in multi-agent setting:} Multi-agent competition can provide a mechanism for driving RL agents to automatically learn increasingly complex behavior \cite{leibo2019autocurricula}. As each agent adapts, it makes the learning problem for the other agent increasingly difficult, leading to the emergence of an automatic curriculum of challenging learning tasks \cite{baker2019emergent,dennis2020emergent,xu2020continual,flet2021adversarially}. For example, \citet{schmidhuber1997s} proposed having two classifiers compete by repeatedly selecting examples which they can classify but which the other cannot. Asymmetric Self Play (ASP) \cite{sukhbaatar2017intrinsic,openai2021asymmetric} rewards one agent, Alice, for executing the shortest trajectory that a second agent, Bob, cannot copy (or reverse). 
% % ASP is limited to training goal-conditioned policies, and is thus less applicable to standard RL tasks where the reward-maximizing states are not known a priori. 
% Similarly to ASP, Adversarial Surprise is formulated as an adversarial game between two policies. However, unlike ASP our method is formulated in terms of general information theoretic quantities which make it more generally applicable. 
% % Adversarial Surprise does not have this limitation, and instead serves as a general algorithm that can speed learning across a variety of contexts.
% For example, we show that ASP can fail to explore stochastic environments, because Alice can easily produce a random goal state which Bob is not able to reproduce. In contrast, AS works well in stochastic environments, outperforming ASP.

\textbf{smirl}
The free energy principle \citep{faraji2018balancing,friston2009free,friston2009reinforcement,friston2016active,ueltzhoffer2018deep}
%%SL.9.30: list the citations in chronological order, with friston2009free first
suggests that biological agents may minimize surprise, or state entropy, in order to remain in safe and stable states. Minimizing
%%SL.9.30: nitpick -- we're a US institution, and we use North American standard English (it's fine to use either one, but it's not fine to mix them, and since most of the paper uses NA standard rather than British standard, better stick to that)
A SMiRL agent trained with this objective learns emergent behaviors to reduce entropy in stochastic environments---such as stable walking robots or playing Tetris---even in the absence of any external reward. However, when applied to partially observed environments, the agent is susceptible to
%%[addressed]MC.5.20: "subject to" --> "susceptible to"
the dark room problem: rather than learning to control the environment, it can simply control its observations by remaining in unsurprising parts of the environment. Or, simply turning to look at a wall. In our method, we build on surprise minimization, incorporating it into a two player game that alleviates this shortcoming.
%%SL.9.30: Generally this paragraph leads well, but I wonder if it can be made a little bit shorter.
